Efficient transmission of measurement data from FPGA to embedded system via Ethernet link

This paper presents a system consisting of the FPGA IP core, the simple network protocol and the Linux device driver, capable of efficient and reliable data transmission from a low resources FPGA chip to the Linux-based embedded computer system, via a private Ethernet network (consisting of a single segment or a few segments connected via an Ethernet switch). The embedded system may optionally process the acquired data, and distribute them further, using standard network protocols. Proposed design targets cost-efficient multichannel data acquisition systems, in which multiple FPGA based front end boards (FEB) should transmit the stream of acquired data to the computer network, responsible for their final processing and archiving. The presented solution allows to minimize the cost of data concentration due to use of inexpensive Ethernet network infrastructure. The work is mainly focused on minimization of resources consumption in the FPGA, and minimization of acknowledge latency in the Linux based system - which allows to achieve high throughput in spite of use of inexpensive FPGA chips with small internal memory.

==> rysunki.src/makefile <==
.SUFFIXES: .svg .dia .fig .eps .figmp .figltx .pdf .jpg .drt .ipe
EPS := $(patsubst %.fig,%.eps,$(wildcard *.fig))\
 $(patsubst %.figmp,%.eps,$(wildcard *.figmp))\
 $(patsubst %.figltx,%.eps,$(wildcard *.figltx))\
 $(patsubst %.pdf,%.eps,$(wildcard *.pdf)) \
 $(patsubst %.svg,%.eps,$(wildcard *.svg)) \
 $(patsubst %.drt,%.eps,$(wildcard *.drt)) \
 $(patsubst %.ipe,%.eps,$(wildcard *.ipe)) \
 $(patsubst %.jpg,%.eps,$(wildcard *.jpg))
DIAEPS := $(patsubst %.dia,%.pdf,$(wildcard *.dia))
  

all: $(EPS) $(DIAEPS)
	echo $(EPS)
	echo Rysunki przetworzone

.jpg.eps: *.jpg
	jpeg2ps $*.jpg > ../rysunki/$*.eps
	ln -s -f ../rysunki.src/$*.jpg ../rysunki/$*.jpg
.fig.eps: *.fig
	fig2dev -L eps $*.fig  ../rysunki/$*.eps
	fig2dev -L pdf $*.fig  ../rysunki/$*.pdf

.pdf.eps: *.pdf
	pdftops -eps $*.pdf  ../rysunki/$*.eps
	ln -s -f $*.pdf ../rysunki/$*.pdf

.figmp.eps: *.figmp
	fig2dev -L mp $*.figmp ../rysunki.tmp/$*.mp
	( cd ../rysunki.tmp ; mpost $*.mp )
	mv ../rysunki.tmp/$*.0 ../rysunki/$*.eps

.figltx.eps: *.figltx
	fig2dev -L pstex -p rysunki/$*.eps $*.figltx ../rysunki/$*.eps
	fig2dev -L pstex_t -p rysunki/$*.eps $*.figltx ../rysunki/$*.tex

.dia.pdf: *.dia
	dia --nosplash -e tmp.fig $*.dia
	fig2dev -j -L pdf tmp.fig ../rysunki/$*.pdf

.drt.eps: *.drt
	drawtiming --output ../rysunki/$*.eps $*.drt

.ipe.eps: *.ipe
	ipetoipe -eps -export $*.ipe ../rysunki/$*.eps

.svg.eps: *.svg
	inkscape -z  -E../rysunki/$*.eps -f $*.svg
#	inkscape -z -d 600 -E../rysunki/$*.eps -f $*.svg
#	inkscape -z --export-ignore-filters -E../rysunki/$*.eps -f $*.svg
	
